ArchGym: An Open-Source Gymnasium for Machine Learning Assisted Architecture Design

Machine learning is a prevalent approach to tame the complexity of design space exploration for domain-specific architectures. Using ML for design space exploration poses challenges. First, it's not straightforward to identify the suitable algorithm from an increasing pool of ML methods. Second, assessing the trade-offs between performance and sample efficiency across these methods is inconclusive. Finally, lack of a holistic framework for fair, reproducible, and objective comparison across these methods hinders progress of adopting ML-aided architecture design space exploration and impedes creating repeatable artifacts. To mitigate these challenges, we introduce ArchGym, an open-source gym and easy-to-extend framework that connects diverse search algorithms to architecture simulators. To demonstrate utility, we evaluate ArchGym across multiple vanilla and domain-specific search algorithms in designing custom memory controller, deep neural network accelerators, and custom SoC for AR/VR workloads, encompassing over 21K experiments. Results suggest that with unlimited samples, ML algorithms are equally favorable to meet user-defined target specification if hyperparameters are tuned; no solution is necessarily better than another (e.g., reinforcement learning vs. Bayesian methods). We coin the term hyperparameter lottery to describe the chance for a search algorithm to find an optimal design provided meticulously selected hyperparameters. The ease of data collection and aggregation in ArchGym facilitates research in ML-aided architecture design space exploration. As a case study, we show this advantage by developing a proxy cost model with an RMSE of 0.61% that offers a 2,000-fold reduction in simulation time. Code and data for ArchGym is available at https://bit.ly/ArchGym.

==> coverletter.tex <==
\onecolumn
\thispagestyle{empty}
\section*{Cover Letter}
\noindent{}We thank the reviewers for their encouraging comments and suggested revisions. We have highlighted the changes in the paper in $\color{magenta}{magenta}$.


\niparagraph{Significance of \ours and contributions.}

\niparagraph{How to extend \ours?}


\niparagraph{Comparison with GAMMA~\cite{gamma}.}


% \paragraph{New evaluations on compatibility of FLAT with SOTA attention-based systems.}
% We added new paragraphs ``FLAT compatibility with sparse-attention accelerators” in \autoref{sec:exp_accel_gpu_attn} to \textit{qualitatively} compare FLAT with SOTA attention-based systems – Sanger~\cite{lu2021sanger} and ELSA~\cite{elsa}. Further, we added \autoref{fig:elsa_cpr} to \textit{quantitatively} compare Sanger v.s. Sanger-FLAT and ELSA v.s. ELSA-FLAT. Our results show both Sanger and ELSA can effectively improve the Baseline (dense attention), and further, they can both leverage FLAT to push their performance since sparse attention is also memory bound.


% \paragraph{New evaluation on protein folding.}
% We thank the reviewers for the suggestions on more in-depth evaluation on protein folding applications.
% % , given that protein folding is a promising applications that would gain benefit from long sequence length. 
% We added the protein folding evaluations presented in the rebuttal into the main paper (\autoref{table:trembl_8k}, \autoref{table:trembl_16k}) and a paragraph called “Case Study on Protein Sequence” in \autoref{sec:evaluations}.

% \paragraph{New evaluation on existing accelerators.}
% We incorporated the FLAT evaluation on Tesla-T4 GPU~\cite{teslaT4} presented in the rebuttal into the main paper (\autoref{table:gpu_sweep_batch}, \autoref{table:gpu_sweep_seq}) and added a paragraph called “FLAT compatibility on GPU” in \autoref{sec:exp_accel_gpu_attn}.

% \paragraph{Differentiation between FLAT and the matrix-matrix fusion in GCNAX~\cite{li2021gcnax} and GRIP~\cite{kiningham2020grip}.}
% We added new related work discussion on GNNs related matrix-matrix fusion accelerators in \autoref{sec:relatedworks}. In brief, there are three main differences: 1) FLAT deals with matrix-Softmax-matrix fusion, which exposes different reuse opportunity to matrix-matrix fusion. 
% 2) Attention, the problem FLAT focuses on, has two activation-activation operations (logit and attend); GNN has one activation-activation and one activation-weight operation. 3) The main challenge of attention comes from \textit{quadratic complexity} of memory and compute, whereas the main challenge of GNNs is the \textit{sparsity} in “aggregate” matrix. In summary, GCNAX and GRIP target GNNs 
% while FLAT targets attentions which face different challenges and expose different optimization opportunities. Fusion as a generic technique, is leveraged across these works, but with different optimizations owing to the difference of the problem space.

% \paragraph{Improve the completeness of related works.}
% Thanks to reviewers’ suggestion, we added GCNAX~\cite{li2021gcnax}, GRIP~\cite{kiningham2020grip}, Sanger~\cite{lu2021sanger}, and SM6~\cite{tambe2021sm6} to make related works more complete.

% \paragraph{Highlight the benefits of common sequences on relatively small buffer sizes.}
% We are aligned with reviewers’ suggestions. We restructured \autoref{sec:exp_util} to focus on the benefit of FLAT at common sequence length (512-token) with relatively small buffer sizes (200KB-20MB) and added \autoref{table:exp_summary} to highlight these benefits. We also incorporated these messages in abstract and \autoref{sec:intro}.

% \paragraph{Motivate on the potentials of long sequences from the algorithmic perspective.}
% We added protein sequencing and text summarization examples in \autoref{sec:intro} to motivate the potential of long sequences.

% \paragraph{Re-plot the figure for better visualization.}
% We used the same set of data to re-plot multiple figures in the papers for better visualization (\autoref{fig:fused_quant}, \autoref{fig:util_cpr_compute_edge}, \autoref{fig:util_cpr_energy_edge},  \autoref{fig:util_cpr_compute_cloud}, \autoref{fig:util_cpr_energy_cloud}, \autoref{fig:latency_ratio}, \autoref{fig:exp_accel_fig}).

% \pagebreak
\twocolumn

==> dse_problem.tex <==
\section{Parameter Design Space Exploration}


The architecture design space exploration corresponds to a class of problems that uses search algorithms to navigate the combinations of all possible valid designs in the large architecture parameter design space. It is classified as a resource allocation problem where the optimal value of each parameter is determined to meet a specific architecture constraint such as area, power, or latency. Typically the architecture parameter space is large and manually searching the whole design space is intractable. Hence, search algorithm are employed to intelligently navigate the large design space.

\textcolor{red}{vj: not clear why we are talking about all this information... also towards the end i feel we repeat more of this from the introduction, same stuff.}

\Fig{fig:arch_dse_problem} depicts the architecture design space exploration problem for different architectures. For example, in \Fig{fig:arch_dse_problem}-a, it depicts the DSE problem from a microarchitecture component (DRAM memory controller). The goal is to find the resource allocation for each parameter that meets a specific target in terms of latency, power, or energy. Likewise, in \Fig{fig:arch_dse_problem}-b and \Fig{fig:arch_dse_problem}-c denotes the DSE problem for DNN hardware accelerator and System-on-Chip (SoC). The table below each architecture template shows the architecture parameter and the search space. For a memory controller, one such parameter can be Scheduler policy which can take one of the possible values from \texttt{<FiFo,FrFcFsGrp, FrFcFs>}. Likewise for DNN accelerator, a control parameter can be number of PEs which can take integer values from \texttt{<14 to 336>} with a step size of \texttt{14}.

The search algorithm iteratively selects the parameter values for a given workload (or set of workloads). The fitness (i.e., how good a particular parameter selection is) of these selections is determined by the architecture cost model. Sometimes, the architecture cost model could be a slow cycle-accurate simulator or a fast analytical model. There is a trade-off between speed and fidelity, which could affect the choice of the search algorithm employed.
%
As the parameter search space increases in complexity (combinatorial explosion), there has been a recent trend of using machine learning algorithms as the search algorithm (See Table~\ref{tab:related-work}) for architecture design space exploration problems. Though ML can be used for many classes of optimization problems, in this work, we limit our study to resource allocation problems. Hence, \textit{our goal is to apply and fairly compare different ML approaches for architecture design space exploration. We also want to understand what are the trade-offs associated with applying different ML algorithms?}
%
To that end, we propose \ours methodology to standardize the ML-driven architecture design space exploration where each ML-based search algorithm uses the same interfaces to solve the architecture design space exploration problem.
